The Colorado Ultraviolet Transit Experiment (CUTE) signal to noise calculator

We present here the signal-to-noise (S/N) calculator developed for the Colorado Ultraviolet Transit Experiment (CUTE) mission. CUTE is a 6U CubeSat operating in the near-ultraviolet (NUV) observing exoplanetary transits to study their upper atmospheres. CUTE was launched into a low-Earth orbit in September 2021 and it is currently gathering scientific data. As part of the S/N calculator, we also present the error propagation for computing transit depth uncertainties starting from the S/N of the original spectroscopic observations. The CUTE S/N calculator is currently extensively used for target selection and scheduling. The modular construction of the CUTE S/N calculator enables its adaptation and can be used also for other missions and instruments.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


